Mid-infrared spectra of T Tauri disks: Modeling the effects of a small inner cavity on CO2 and H2O emission

[Abridged] The inner few AU of disks around young stars are best probed in the infrared. The James Webb Space Telescope (JWST) is now starting to characterize the chemistry of these regions in unprecedented detail. One peculiar subset of sources are the so-called ``CO2-only sources'', in which only a strong 15 $\mu$m CO2 feature was detected in the spectrum. One scenario that could explain the weak emission from H2O is the presence of a small, inner cavity in the disk. If this cavity were to extend past the H2O snowline, but not past the CO2 snowline, this could strongly suppress the H2O line flux w.r.t. that of CO2. In this work, we aim to test the validity of this statement. Using the thermo-chemical code Dust And LInes (DALI), we created a grid of T Tauri disk models with an inner cavity, meaning we fully depleted the inner region of the disk in gas and dust starting from the dust sublimation radius and ranging until a certain cavity radius. We present the evolution of the CO2 and H2O spectra of a disk with inner cavity size, showing that, when a large-enough cavity is introduced, a spectrum that was initially dominated by H2O lines can become CO2-dominated instead. However, the cavity size needed for this is around 4-5 AU, exceeding the nominal position of the CO2 snowline in a full disk. The cause of this is most likely the alteration of the thermal structure by the cavity, which pushes the snowlines outward. Alternative explanations for bright CO2 emission are also briefly discussed. Our modeling work shows that it is possible for the presence of a small inner cavity to explain strong CO2 emission in a spectrum. However, the cavity needed to do so is larger than what was initially expected. As such, this scenario will be easier to test with sufficiently high angular resolution (millimeter) observations.

==> dem.tex <==
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Example below of non-structurated natbib references  
% To use the v8.3 macros with this form of composition of bibliography, 
% the option "bibyear" should be added to the command line 
% "\documentclass[bibyear]{aa}".
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{thebibliography}{}

%   \bibitem[1966]{baker} Baker, N. 1966,
%       in Stellar Evolution,
%       ed.\ R. F. Stein,\& A. G. W. Cameron
%       (Plenum, New York) 333

%    \bibitem[1988]{balluch} Balluch, M. 1988,
%       A\&A, 200, 58

%    \bibitem[1980]{cox} Cox, J. P. 1980,
%       Theory of Stellar Pulsation
%       (Princeton University Press, Princeton) 165

%    \bibitem[1969]{cox69} Cox, A. N.,\& Stewart, J. N. 1969,
%       Academia Nauk, Scientific Information 15, 1

%    \bibitem[1980]{mizuno} Mizuno H. 1980,
%       Prog. Theor. Phys., 64, 544
   
%    \bibitem[1987]{tscharnuter} Tscharnuter W. M. 1987,
%       A\&A, 188, 55
  
%    \bibitem[1992]{terlevich} Terlevich, R. 1992, in ASP Conf. Ser. 31, 
%       Relationships between Active Galactic Nuclei and Starburst Galaxies, 
%       ed. A. V. Filippenko, 13

%    \bibitem[1980a]{yorke80a} Yorke, H. W. 1980a,
%       A\&A, 86, 286

%    \bibitem[1997]{zheng} Zheng, W., Davidsen, A. F., Tytler, D. \& Kriss, G. A.
%       1997, preprint
% \end{thebibliography}
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Examples for figures using graphicx
% A guide "Using Imported Graphics in LaTeX2e"  (Keith Reckdahl)
% is available on a lot of LaTeX public servers or ctan mirrors.
% The file is : epslatex.pdf 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %-------------------------------------------------------------
% %                 A figure as large as the width of the column
% %-------------------------------------------------------------
%    \begin{figure}
%    \centering
%    \includegraphics[width=\hsize]{empty.eps}
%       \caption{Vibrational stability equation of state
%                $S_{\mathrm{vib}}(\lg e, \lg \rho)$.
%                $>0$ means vibrational stability.
%               }
%          \label{FigVibStab}
%    \end{figure}
% %
% %-------------------------------------------------------------
% %                                    One column rotated figure
% %-------------------------------------------------------------
%    \begin{figure}
%    \centering
%    \includegraphics[angle=-90,width=3cm]{empty.eps}
%       \caption{Vibrational stability equation of state
%                $S_{\mathrm{vib}}(\lg e, \lg \rho)$.
%                $>0$ means vibrational stability.
%               }
%          \label{FigVibStab}
%    \end{figure}
% %
% %-------------------------------------------------------------
% %                        Figure with caption on the right side 
% %-------------------------------------------------------------
%    \begin{figure}
%    \sidecaption
%    \includegraphics[width=3cm]{empty.eps}
%       \caption{Vibrational stability equation of state
%                $S_{\mathrm{vib}}(\lg e, \lg \rho)$.
%                $>0$ means vibrational stability.
%               }
%          \label{FigVibStab}
%    \end{figure}
% %
% %-------------------------------------------------------------
% %                                Figure with a new BoundingBox 
% %-------------------------------------------------------------
%    \begin{figure}
%    \centering
%    \includegraphics[bb=10 20 100 300,width=3cm,clip]{empty.eps}
%       \caption{Vibrational stability equation of state
%                $S_{\mathrm{vib}}(\lg e, \lg \rho)$.
%                $>0$ means vibrational stability.
%               }
%          \label{FigVibStab}
%    \end{figure}
% %
% %-------------------------------------------------------------
% %                                      The "resizebox" command 
% %-------------------------------------------------------------
%    \begin{figure}
%    \resizebox{\hsize}{!}
%             {\includegraphics[bb=10 20 100 300,clip]{empty.eps}
%       \caption{Vibrational stability equation of state
%                $S_{\mathrm{vib}}(\lg e, \lg \rho)$.
%                $>0$ means vibrational stability.
%               }
%          \label{FigVibStab}
%    \end{figure}
% %
% %-------------------------------------------------------------
% %                                             Two column Figure 
% %-------------------------------------------------------------
%    \begin{figure*}
%    \resizebox{\hsize}{!}
%             {\includegraphics[bb=10 20 100 300,clip]{empty.eps}
%       \caption{Vibrational stability equation of state
%                $S_{\mathrm{vib}}(\lg e, \lg \rho)$.
%                $>0$ means vibrational stability.
%               }
%          \label{FigVibStab}
%    \end{figure*}
% %
% %-------------------------------------------------------------
% %                                             Simple A&A Table
% %-------------------------------------------------------------
% %
% \begin{table}
% \caption{Nonlinear Model Results}             % title of Table
% \label{table:1}      % is used to refer this table in the text
% \centering                          % used for centering table
% \begin{tabular}{c c c c}        % centered columns (4 columns)
% \hline\hline                 % inserts double horizontal lines
% HJD & $E$ & Method\#2 & Method\#3 \\    % table heading 
% \hline                        % inserts single horizontal line
%    1 & 50 & $-837$ & 970 \\      % inserting body of the table
%    2 & 47 & 877    & 230 \\
%    3 & 31 & 25     & 415 \\
%    4 & 35 & 144    & 2356 \\
%    5 & 45 & 300    & 556 \\ 
% \hline                                   %inserts single line
% \end{tabular}
% \end{table}
% %
% %-------------------------------------------------------------
% %                                             Two column Table 
% %-------------------------------------------------------------
% %
% \begin{table*}
% \caption{Nonlinear Model Results}             
% \label{table:1}      
% \centering          
% \begin{tabular}{c c c c l l l }     % 7 columns 
% \hline\hline       
%                       % To combine 4 columns into a single one 
% HJD & $E$ & Method\#2 & \multicolumn{4}{c}{Method\#3}\\ 
% \hline                    
%    1 & 50 & $-837$ & 970 & 65 & 67 & 78\\  
%    2 & 47 & 877    & 230 & 567& 55 & 78\\
%    3 & 31 & 25     & 415 & 567& 55 & 78\\
%    4 & 35 & 144    & 2356& 567& 55 & 78 \\
%    5 & 45 & 300    & 556 & 567& 55 & 78\\
% \hline                  
% \end{tabular}
% \end{table*}
% %
% %-------------------------------------------------------------
% %                                          Table with notes 
% %-------------------------------------------------------------
% %
% % A single note
% \begin{table}
% \caption{\label{t7}Spectral types and photometry for stars in the
%   region.}
% \centering
% \begin{tabular}{lccc}
% \hline\hline
% Star&Spectral type&RA(J2000)&Dec(J2000)\\
% \hline
% 69           &B1\,V     &09 15 54.046 & $-$50 00 26.67\\
% 49           &B0.7\,V   &*09 15 54.570& $-$50 00 03.90\\
% LS~1267~(86) &O8\,V     &09 15 52.787&11.07\\
% 24.6         &7.58      &1.37 &0.20\\
% \hline
% LS~1262      &B0\,V     &09 15 05.17&11.17\\
% MO 2-119     &B0.5\,V   &09 15 33.7 &11.74\\
% LS~1269      &O8.5\,V   &09 15 56.60&10.85\\
% \hline
% \end{tabular}
% \tablefoot{The top panel shows likely members of Pismis~11. The second
% panel contains likely members of Alicante~5. The bottom panel
% displays stars outside the clusters.}
% \end{table}
% %
% % More notes
% %
% \begin{table}
% \caption{\label{t7}Spectral types and photometry for stars in the
%   region.}
% \centering
% \begin{tabular}{lccc}
% \hline\hline
% Star&Spectral type&RA(J2000)&Dec(J2000)\\
% \hline
% 69           &B1\,V     &09 15 54.046 & $-$50 00 26.67\\
% 49           &B0.7\,V   &*09 15 54.570& $-$50 00 03.90\\
% LS~1267~(86) &O8\,V     &09 15 52.787&11.07\tablefootmark{a}\\
% 24.6         &7.58\tablefootmark{1}&1.37\tablefootmark{a}   &0.20\tablefootmark{a}\\
% \hline
% LS~1262      &B0\,V     &09 15 05.17&11.17\tablefootmark{b}\\
% MO 2-119     &B0.5\,V   &09 15 33.7 &11.74\tablefootmark{c}\\
% LS~1269      &O8.5\,V   &09 15 56.60&10.85\tablefootmark{d}\\
% \hline
% \end{tabular}
% \tablefoot{The top panel shows likely members of Pismis~11. The second
% panel contains likely members of Alicante~5. The bottom panel
% displays stars outside the clusters.\\
% \tablefoottext{a}{Photometry for MF13, LS~1267 and HD~80077 from
% Dupont et al.}
% \tablefoottext{b}{Photometry for LS~1262, LS~1269 from
% Durand et al.}
% \tablefoottext{c}{Photometry for MO2-119 from
% Mathieu et al.}
% }
% \end{table}
% %
% %-------------------------------------------------------------
% %                                       Table with references 
% %-------------------------------------------------------------
% %
% \begin{table*}[h]
%  \caption[]{\label{nearbylistaa2}List of nearby SNe used in this work.}
% \begin{tabular}{lccc}
%  \hline \hline
%   SN name &
%   Epoch &
%  Bands &
%   References \\
%  &
%   (with respect to $B$ maximum) &
%  &
%  \\ \hline
% 1981B   & 0 & {\it UBV} & 1\\
% 1986G   &  $-$3, $-$1, 0, 1, 2 & {\it BV}  & 2\\
% 1989B   & $-$5, $-$1, 0, 3, 5 & {\it UBVRI}  & 3, 4\\
% 1990N   & 2, 7 & {\it UBVRI}  & 5\\
% 1991M   & 3 & {\it VRI}  & 6\\
% \hline
% \noalign{\smallskip}
% \multicolumn{4}{c}{ SNe 91bg-like} \\
% \noalign{\smallskip}
% \hline
% 1991bg   & 1, 2 & {\it BVRI}  & 7\\
% 1999by   & $-$5, $-$4, $-$3, 3, 4, 5 & {\it UBVRI}  & 8\\
% \hline
% \noalign{\smallskip}
% \multicolumn{4}{c}{ SNe 91T-like} \\
% \noalign{\smallskip}
% \hline
% 1991T   & $-$3, 0 & {\it UBVRI}  &  9, 10\\
% 2000cx  & $-$3, $-$2, 0, 1, 5 & {\it UBVRI}  & 11\\ %
% \hline
% \end{tabular}
% \tablebib{(1)~\citet{branch83};
% (2) \citet{phillips87}; (3) \citet{barbon90}; (4) \citet{wells94};
% (5) \citet{mazzali93}; (6) \citet{gomez98}; (7) \citet{kirshner93};
% (8) \citet{patat96}; (9) \citet{salvo01}; (10) \citet{branch03};
% (11) \citet{jha99}.
% }
% \end{table*}
% %-------------------------------------------------------------
% %                      A rotated Two column Table in landscape  
% %-------------------------------------------------------------
% \begin{sidewaystable*}
% \caption{Summary for ISOCAM sources with mid-IR excess 
% (YSO candidates).}\label{YSOtable}
% \centering
% \begin{tabular}{crrlcl} 
% \hline\hline             
% ISO-L1551 & $F_{6.7}$~[mJy] & $\alpha_{6.7-14.3}$ 
% & YSO type$^{d}$ & Status & Comments\\
% \hline
%   \multicolumn{6}{c}{\it New YSO candidates}\\ % To combine 6 columns into a single one
% \hline
%   1 & 1.56 $\pm$ 0.47 & --    & Class II$^{c}$ & New & Mid\\
%   2 & 0.79:           & 0.97: & Class II ?     & New & \\
%   3 & 4.95 $\pm$ 0.68 & 3.18  & Class II / III & New & \\
%   5 & 1.44 $\pm$ 0.33 & 1.88  & Class II       & New & \\
% \hline
%   \multicolumn{6}{c}{\it Previously known YSOs} \\
% \hline
%   61 & 0.89 $\pm$ 0.58 & 1.77 & Class I & \object{HH 30} & Circumstellar disk\\
%   96 & 38.34 $\pm$ 0.71 & 37.5& Class II& MHO 5          & Spectral type\\
% \hline
% \end{tabular}
% \end{sidewaystable*}
% %-------------------------------------------------------------
% %                      A rotated One column Table in landscape  
% %-------------------------------------------------------------
% \begin{sidewaystable}
% \caption{Summary for ISOCAM sources with mid-IR excess 
% (YSO candidates).}\label{YSOtable}
% \centering
% \begin{tabular}{crrlcl} 
% \hline\hline             
% ISO-L1551 & $F_{6.7}$~[mJy] & $\alpha_{6.7-14.3}$ 
% & YSO type$^{d}$ & Status & Comments\\
% \hline
%   \multicolumn{6}{c}{\it New YSO candidates}\\ % To combine 6 columns into a single one
% \hline
%   1 & 1.56 $\pm$ 0.47 & --    & Class II$^{c}$ & New & Mid\\
%   2 & 0.79:           & 0.97: & Class II ?     & New & \\
%   3 & 4.95 $\pm$ 0.68 & 3.18  & Class II / III & New & \\
%   5 & 1.44 $\pm$ 0.33 & 1.88  & Class II       & New & \\
% \hline
%   \multicolumn{6}{c}{\it Previously known YSOs} \\
% \hline
%   61 & 0.89 $\pm$ 0.58 & 1.77 & Class I & \object{HH 30} & Circumstellar disk\\
%   96 & 38.34 $\pm$ 0.71 & 37.5& Class II& MHO 5          & Spectral type\\
% \hline
% \end{tabular}
% \end{sidewaystable}
% %
% %-------------------------------------------------------------
% %                              Table longer than a single page  
% %-------------------------------------------------------------
% % All long tables will be placed automatically at the end of the document
% %
% \longtab{
% \begin{longtable}{lllrrr}
% \caption{\label{kstars} Sample stars with absolute magnitude}\\
% \hline\hline
% Catalogue& $M_{V}$ & Spectral & Distance & Mode & Count Rate \\
% \hline
% \endfirsthead
% \caption{continued.}\\
% \hline\hline
% Catalogue& $M_{V}$ & Spectral & Distance & Mode & Count Rate \\
% \hline
% \endhead
% \hline
% \endfoot
% %%
% Gl 33    & 6.37 & K2 V & 7.46 & S & 0.043170\\
% Gl 66AB  & 6.26 & K2 V & 8.15 & S & 0.260478\\
% Gl 68    & 5.87 & K1 V & 7.47 & P & 0.026610\\
%          &      &      &      & H & 0.008686\\
% Gl 86 
% \footnote{Source not included in the HRI catalog. See Sect.~5.4.2 for details.}
%          & 5.92 & K0 V & 10.91& S & 0.058230\\
% \end{longtable}
% }
% %
% %-------------------------------------------------------------
% %                              Table longer than a single page
% %                                            and in landscape, 
% %                    in the preamble, use: \usepackage{lscape}
% %-------------------------------------------------------------

% % All long tables will be placed automatically at the end of the document
% %
% \longtab{
% \begin{landscape}
% \begin{longtable}{lllrrr}
% \caption{\label{kstars} Sample stars with absolute magnitude}\\
% \hline\hline
% Catalogue& $M_{V}$ & Spectral & Distance & Mode & Count Rate \\
% \hline
% \endfirsthead
% \caption{continued.}\\
% \hline\hline
% Catalogue& $M_{V}$ & Spectral & Distance & Mode & Count Rate \\
% \hline
% \endhead
% \hline
% \endfoot
% %%
% Gl 33    & 6.37 & K2 V & 7.46 & S & 0.043170\\
% Gl 66AB  & 6.26 & K2 V & 8.15 & S & 0.260478\\
% Gl 68    & 5.87 & K1 V & 7.47 & P & 0.026610\\
%          &      &      &      & H & 0.008686\\
% Gl 86
% \footnote{Source not included in the HRI catalog. See Sect.~5.4.2 for details.}
%          & 5.92 & K0 V & 10.91& S & 0.058230\\
% \end{longtable}
% \end{landscape}
% }
% %
% %-------------------------------------------------------------
% %               Appendices have to be placed at the end, after
% %                                        \end{thebibliography}
% %-------------------------------------------------------------
% \end{thebibliography}

% \begin{appendix} %First appendix
% \section{Background galaxy number counts and shear noise-levels}
% Because the optical images used in this analysis...
% \begin{figure*}%f1
% \includegraphics[width=10.9cm]{1787f23.eps}
% \caption{Shown in greyscale is a...}
% \label{cl12301}
% \end{figure*}

% In this case....
% \begin{figure*}
% \centering
% \includegraphics[width=16.4cm,clip]{1787f24.ps}
% \caption{Plotted above...}
% \label{appfig}
% \end{figure*}

% Because the optical images...

% \section{Title of Second appendix.....} %Second appendix
% These studies, however, have faced...
% \begin{table}
% \caption{Complexes characterisation.}\label{starbursts}
% \centering
% \begin{tabular}{lccc}
% \hline \hline
% Complex & $F_{60}$ & 8.6 &  No. of  \\
% ...
% \hline
% \end{tabular}
% \end{table}

% The second method produces...
% \end{appendix}
% %
% %
% \end{document}

% %
% %-------------------------------------------------------------
% %          For the appendices, table longer than a single page
% %-------------------------------------------------------------

% % Table will be print automatically at the end of the document, 
% % after the whole appendices

% \begin{appendix} %First appendix
% \section{Background galaxy number counts and shear noise-levels}

% % In the appendices do not forget to put the counter of the table 
% % as an option

% \longtab[1]{
% \begin{longtable}{lrcrrrrrrrrl}
% \caption{Line data and abundances ...}\\
% \hline
% \hline
% Def & mol & Ion & $\lambda$ & $\chi$ & $\log gf$ & N & e &  rad & $\delta$ & $\delta$ 
% red & References \\
% \hline
% \endfirsthead
% \caption{Continued.} \\
% \hline
% Def & mol & Ion & $\lambda$ & $\chi$ & $\log gf$ & B & C &  rad & $\delta$ & $\delta$ 
% red & References \\
% \hline
% \endhead
% \hline
% \endfoot
% \hline
% \endlastfoot
% A & CH & 1 &3638 & 0.002 & $-$2.551 &  &  &  & $-$150 & 150 &  Jorgensen et al. (1996) \\                    
% \end{longtable}
% }% End longtab
% \end{appendix}

% %-------------------------------------------------------------
% %                   For appendices and landscape, large table:
% %                    in the preamble, use: \usepackage{lscape}
% %-------------------------------------------------------------

% \begin{appendix} %First appendix
% %
% \longtab[1]{
% \begin{landscape}
% \begin{longtable}{lrcrrrrrrrrl}
% ...
% \end{longtable}
% \end{landscape}
% }% End longtab
% \end{appendix}

% %%%% End of aa.dem

